Learning-Enhanced Reduce-Repair-Refine-Optimize Framework for Real-Time Train Platforming

Real-time train platforming under disruptions requires rapid revision of routing, platforming, and timing decisions. Dense traffic and shared infrastructure create tightly coupled conflicts, making real-time optimization computationally demanding. This paper proposes a learning-enhanced Reduce-Repair-Refine-Optimize framework that reduces and selectively relaxes the routing search space to balance computational efficiency, feasibility, and solution quality. The reduction stage constructs a restricted MILP by fixing selected routing decisions using route-specific predictive models and thresholds, thereby accounting for heterogeneity across routes. Two adaptive mechanisms subsequently modify the reduced search space: repair selectively releases route fixings to restore feasibility, while refinement releases additional fixings to recover routing alternatives and improve solution quality without reverting to the unrestricted problem. Computational experiments on real-life disrupted station-area instances show that the framework matches or improves upon a recent rTPP heuristic in more than 80% of instances within 60~s. Under the common 180~s budget, the framework obtains strictly better terminal incumbents than the unrestricted MILP in 56.7% of all instances and 77.4% of hard instances. Moreover, it obtains better terminal incumbents than an otherwise identical variant without refinement in 71.9% of hard instances. The results demonstrate that learning-based search-space reduction is most effective when the reduced search space remains adaptable during optimization, enabling high-quality feasible solutions within the real-time computation budget.

==> Tables/app_notation_pars.tex <==
\begin{table}[htbp]
\captionsetup{singlelinecheck=false, justification=raggedright}
\caption{Notation of sets and parameters used in the MILP.}
\label{tab:notation_pars}
\footnotesize
\renewcommand{\arraystretch}{1.15}
\begin{tabularx}{\textwidth}{@{}p{0.25\textwidth}X@{}}
\toprule
\textbf{Notation} & \textbf{Description} \\
\midrule

\multicolumn{2}{@{}l}{\textbf{Sets}} \\
$\mathbf{T}$ & Scheduled trains \\
$\mathbf{T^o}, \mathbf{T^e}$ & Originating and terminating trains \\
$\mathbf{\tilde{T}}, \mathbf{\bar{T}}$ & Train pairs running in the same / opposing direction that may generate conflicts \\
$\mathbf{Q}$ & Running directions of trains \\
$R_t^{\text{in}}, R_t^{\text{out}}$ & Feasible inbound and outbound routes for train $t$ \\
$\mathbf{R^x}$ & Dummy routes used for cancellation \\
$\mathbf{P}, \mathbf{P_t}$ & Platforms in the station area, feasible platforms for train $t$ \\

\midrule
\multicolumn{2}{@{}l}{\textbf{Parameters}} \\
$\lambda_X, \lambda_D, \lambda_P, \lambda_R \in \mathbb{R}_{\ge 0}$ & Weights of the cost components in the objective function \\
$q_t$ & Running direction of train $t$ \\
$\tau^{\text{in}}_t, \tau^{\text{out}}_t$ & Inbound and outbound running time of train $t$ \\
$p(r)$ & Platform associated with route $r$ \\
$\mu_{rr'}$ & 1 if inbound routes $r$ and $r'$ share the same entry infrastructure element; 0 otherwise \\
$\pi_{rr'}$ & 1 if inbound routes $r$ and $r'$ use the same platform; 0 otherwise \\
$\nu_{rr'}$ & 1 if inbound routes $r$ and $r'$ share a non-entry infrastructure element; 0 otherwise \\
$\omega_{rr'}$ & 1 if outbound routes $r$ and $r'$ have at least one common infrastructure element; 0 otherwise \\
$\zeta_{rr'}$ & 1 if opposing routes $r$ and $r'$ share at least one common infrastructure element; 0 otherwise \\
$\eta_{rr'}$ & 1 if opposing routes $r$ and $r'$ share only the platform; 0 otherwise \\
$\hat{\alpha}^r_t$ & 1 if train $t$ is nominally assigned to inbound route $r$; 0 otherwise \\
$\hat{\beta}^r_t$ & 1 if train $t$ is nominally assigned to outbound route $r$; 0 otherwise \\
$\hat{p}_t$ & Nominally assigned platform of train $t$ \\
$\hat{a}^s_t, \hat{d}^s_t$ & Nominal scheduled arrival and departure time at the station boundary \\
$\hat{a}^p_t, \hat{d}^p_t$ & Nominal scheduled arrival and departure time at the platform \\
$\hat{w}^s_t, \hat{w}^p_t$ & Nominal scheduled waiting time at home signal / dwell time at platform \\
$\bar{w}^s, \bar{w}^{p}$ & Maximum allowed waiting and dwell time \\
$M$ & Sufficiently large constant \\

\bottomrule
\end{tabularx}
\end{table}


==> Tables/app_notation_vars.tex <==
\begin{table}[htbp]
\captionsetup{singlelinecheck=false, justification=raggedright}
\caption{Notation of decision variables in the MILP.}
\label{tab:notation_vars}
\footnotesize
\renewcommand{\arraystretch}{1.15}
\begin{tabularx}{\textwidth}{@{}p{0.12\textwidth}X@{}}
\toprule
\textbf{Notation} & \textbf{Description} \\
\midrule

\multicolumn{2}{@{}l}{\textbf{Binary decision variables}} \\
$\delta^{\text{in}}_t, \delta^{\text{out}}_t$ & Indicator for inbound / outbound route change of train $t$ \\
$\alpha^{r}_{t}$ & 1 if train $t$ is assigned to inbound route $r$; 0 otherwise \\
$\beta^{r}_{t}$ & 1 if train $t$ is assigned to outbound route $r$; 0 otherwise \\
$\gamma^{r}_{t}$ & 1 if train $t$ is canceled and assigned to dummy route $r$; 0 otherwise \\
$y_{tt'}$ & 1 if train $t$ enters the station area before train $t'$ on the same entry infrastructure element; 0 otherwise \\
$z_{tt'}$ & 1 if train $t$ departs from the same platform before train $t'$; 0 otherwise \\

\midrule
\multicolumn{2}{@{}l}{\textbf{Continuous decision variables}} \\
$a^s_t, d^s_t$ & Revised arrival and departure time of train $t$ at the station boundary \\
$a^p_t, d^p_t$ & Revised arrival and departure time of train $t$ at the platform \\
$\Delta p_t$ & Change in platform assignment for train $t$ \\
$\Delta w^s_t, \Delta w^p_t$ & Change in waiting time at home signal / dwell time at platform for train $t$ \\

\bottomrule
\end{tabularx}
\end{table}

